eFontes. Part of Speech Tagging and Lemmatization of Medieval Latin Texts.A Cross-Genre Survey

This study introduces the eFontes models for automatic linguistic annotation of Medieval Latin texts, focusing on lemmatization, part-of-speech tagging, and morphological feature determination. Using the Transformers library, these models were trained on Universal Dependencies (UD) corpora and the newly developed eFontes corpus of Polish Medieval Latin. The research evaluates the models' performance, addressing challenges such as orthographic variations and the integration of Latinized vernacular terms. The models achieved high accuracy rates: lemmatization at 92.60%, part-of-speech tagging at 83.29%, and morphological feature determination at 88.57%. The findings underscore the importance of high-quality annotated corpora and propose future enhancements, including extending the models to Named Entity Recognition.

==> tables/UD_data_old.tex <==
\begin{table*}[ht]
\begin{center}
\small
\begin{tabular}{@{}llrrr@{}}

      \toprule
      Corpus&Type&Tokens&Sentences&Avg\\
      \midrule
      ITTB & Medieval Latin - Thomas Aquinas & 390 819 & 22 775 & 17.16\\
      PROIEL & Vulgate New Testament \& 1st century BC Roman Empire & 177 558 & 16 196 & 10.96\\
     Perseus & Ancient Latin, multiple authors & 18 425 & 1 334 & 13.81\\
     UDante & Latin Dante Alighieri & 30 566 & 926 & 33.01\\
     LLCT & 19th century Italian Latin & 390 819 & 7 289 & 26.64\\
    \bottomrule

\end{tabular}
\caption{Number of tokens, sentences and average number of tokens in a sentence in Universal Dependencies corpora used in the scenarios involving UD data.}
 \end{center}
\end{table*}

==> tables/UD_h_spelling.tex <==
\begin{table}[!htbp]
\small
\centering
\begin{tabular}{cc|ccccc}
 \toprule
Position &  & UDante & LLCT & ITTB & Perseus & PROIEL\\[0pt]
\midrule
initial & hV & hostium : ostium & homne : omnis & humorum : umor & & have : ave\\[0pt]
 & Ch & thonus : tonus & Chunimundo : Cunimundus &  &  & \\[0pt]
middle & VhV &  & Danihel : Daniel &  &  & Israhel : Israel\\[0pt]
 & Ch & nothus : notus & schabinus : scabinus &  &  & \\[0pt]
 \bottomrule
\end{tabular}
    \caption{Evidence for \textit{h} spelling in the UD corpora.}
    \label{tab:ud_h_spelling}
\end{table}


==> tables/allUD_finetuned_on_efontes.tex <==
\begin{table*}[ht]
\tiny
    \begin{center}
    \begin{tabular}{|c|ccc|ccc|ccc|ccc|ccc|}
        \hline
        \multirow{2}{*}{Corpus} & \multicolumn{3}{c|}{Proceedings} & \multicolumn{3}{c|}{Science}& \multicolumn{3}{c|}{Annals}& \multicolumn{3}{c|}{Biography} & \multicolumn{3}{c|}{Normative}\\
        \cline{2-16}
        & UPOS & UFeats & Lemma & UPOS & UFeats & Lemma & UPOS & UFeats & Lemma & UPOS & UFeats & Lemma & UPOS & UFeats & Lemma \\
        \hline
        baseline eFontes & 91.63 & 86.67 & 81.69 & 79.21 & 77.48 & 80.53 & 95.98 & 80.78 & 87.04 & 95.43 & 82.06 & 80.75 & 95.81 & 81.53 & 85.05\\
        eFontes fine-tuned & \textbf{94.97} & \textbf{87.67} & \textbf{83.17} & \textbf{79.61} & \underline{78.60} & \underline{96.35} & \textbf{96.20} & \textbf{81.45} & \textbf{86.82} & \textbf{96.10} & \textbf{83.86} & \textbf{88.12} & \textbf{96.10} & \textbf{84.86} & \textbf{88.37}\\
        all UD corpora & 93.18 & 67.12 & 79.82 & \underline{75.35} & 51.88 & \textbf{96.45} & 86.15 & 59.11 & 82.79 & 90.19 & 52.85 & 86.14 & \underline{92.04} & 50.32 & 85.81\\
        UD + ITTB & 91.06 & 70.62 & 79.03 & 74.65 & 48.78 & 95.44 & 87.15 & 31.40 & \underline{85.14} & 89.58 & 32.02 & \underline{87.48} & 91.66 & 67.96 & 85.85\\
        UD + LLCT & 91.06 & 70.62 & 78.95 & 75.15 & 68.51 & 95.94 & 86.93 & 70.50 & 83.46 & 89.87 & 69.84 & 86.65 & 91.66 & 67.96 & \underline{86.26}\\
        UD + UDante & \underline{93.42} & 37.67 & \underline{80.28} & 74.65 & 51.83 & 95.23 & \underline{88.60} & 32.18 & 83.91 & 90.20 & 33.56 & 86.30 & 91.69 & 34.44 & 85.08\\
        UD + Perseus & 93.35 & 73.26 & 78.99 & 75.30 & 61.26 & 94.73 & 86.48 & 71.06 & 81.68 & \underline{90.34} & 72.68 & 84.42 & 92.01 & 69.87 & 83.74\\
        UD + PROIEL & 80.04 & \underline{74.23} & 79.87 & 61.56 & \textbf{87.37} & 94.12 & 75.08 & \underline{76.09} & 81.79 & 77.34 & \underline{75.78} & 85.10 & 79.46 & \underline{71.95} & 84.73\\
        \hline
    \end{tabular}
    \caption{Testing model fine-tuned on specific UD corpus with eFontes data}
    \end{center}
\end{table*}


==> tables/allUD_finetuned_on_efontes_col.tex <==
\begin{table*}[!htb]
\centering
\tiny
\begin{tabular}{lccccccccccccccc}
\toprule
 & \multicolumn{3}{c}{Proceedings} & \multicolumn{3}{c}{Science} & \multicolumn{3}{c}{Annals} & \multicolumn{3}{c}{Biography} & \multicolumn{3}{c}{Normative} \\
 & UPOS & UFeats & Lemma & UPOS & UFeats & Lemma & UPOS & UFeats & Lemma & UPOS & UFeats & Lemma & UPOS & UFeats & Lemma \\
\midrule
baseline & 91.63 & 86.67 & 81.69 & 79.21 & 77.48 & 80.53 & 95.98 & 80.78 & \color{black} {\cellcolor[HTML]{B6E880}} 87.04 & 95.43 & 82.06 & 80.75 & 95.81 & 81.53 & 85.05\\
UD all & 93.18 & 67.12 & 79.82 & 75.35 & 51.88 & \color{black} {\cellcolor[HTML]{B6E880}} 96.45 & 86.15 & 59.11 & 82.79 & 90.19 & 52.85 & 86.14 & 92.04 & 50.32 & 85.81 \\
UD + ITTB & 91.06 & 70.62 & 79.03 & 74.65 & \color{black} {\cellcolor[HTML]{EF553B}} 48.78 & 95.44 & 87.15 & \color{black} {\cellcolor[HTML]{EF553B}} 31.40 & 85.14 & 89.58 & \color{black} {\cellcolor[HTML]{EF553B}} 32.02 & 87.48 & 91.66 & 67.96 & 85.85 \\
UD + LLCT & 91.06 & 70.62 & \color{black} {\cellcolor[HTML]{EF553B}} 78.95 & 75.15 & 68.51 & 95.94 & 86.93 & 70.50 & 83.46 & 89.87 & 69.84 & 86.65 & 91.66 & 67.96 & 86.26 \\
UD + Perseus & 93.35 & 73.26 & 78.99 & 75.30 & 61.26 & 94.73 & 86.48 & 71.06 & \color{black} {\cellcolor[HTML]{EF553B}} 81.68 & 90.34 & 72.68 & \color{black} {\cellcolor[HTML]{EF553B}} 84.42 & 92.01 & 69.87 & \color{black} {\cellcolor[HTML]{EF553B}} 83.74 \\
UD + PROIEL & \color{black} {\cellcolor[HTML]{EF553B}} 80.04 & 74.23 & 79.87 & \color{black} {\cellcolor[HTML]{EF553B}} 61.56 & \color{black} {\cellcolor[HTML]{B6E880}} 87.37 & \color{black} {\cellcolor[HTML]{EF553B}} 94.12 & \color{black} {\cellcolor[HTML]{EF553B}} 75.08 & 76.09 & 81.79 & \color{black} {\cellcolor[HTML]{EF553B}} 77.34 & 75.78 & 85.10 & \color{black} {\cellcolor[HTML]{EF553B}} 79.46 & 71.95 & 84.73 \\
UD + UDante & 93.42 & \color{black} {\cellcolor[HTML]{EF553B}} 37.67 & 80.28 & 74.65 & 51.83 & 95.23 & 88.60 & 32.18 & 83.91 & 90.20 & 33.56 & 86.30 & 91.69 & \color{black} {\cellcolor[HTML]{EF553B}} 34.44 & 85.08 \\
UD + eFontes & \color{black} {\cellcolor[HTML]{B6E880}} 94.97 & \color{black} {\cellcolor[HTML]{B6E880}} 87.67 & \color{black} {\cellcolor[HTML]{B6E880}} 83.17 & \color{black} {\cellcolor[HTML]{B6E880}} 79.61 & 78.60 & 96.35 & \color{black} {\cellcolor[HTML]{B6E880}} 96.20 & \color{black} {\cellcolor[HTML]{B6E880}} 81.45 & 86.82 & \color{black} {\cellcolor[HTML]{B6E880}} 96.10 & \color{black} {\cellcolor[HTML]{B6E880}} 83.86 & \color{black} {\cellcolor[HTML]{B6E880}} 88.12 & \color{black} {\cellcolor[HTML]{B6E880}} 96.10 & \color{black} {\cellcolor[HTML]{B6E880}} 84.86 & \color{black} {\cellcolor[HTML]{B6E880}} 88.37 \\
\hline
\end{tabular}
\label{tab:full}
\caption{The results of the various training scenarios described in Section \ref{sec:system}. Green color indicates the best result, while red indicates the worse result for a given subcorpus-task combination. The results involving eFontes data (\textit{baseline} and \textit{UD + eFontes}) are reported for the cross-validation scheme, i.e. the evaluated model was trained on the data excluding the testing subcorpus. For the other scenarios for each task only one model was trained and the results show its performance for the different subcorpora.}
\end{table*}


==> tables/allUD_on_efontes.tex <==
\begin{table}[!ht]
\begin{center}
\begin{tabular}{@{}lrrr@{}}

      \toprule
      Genre&UPOS&UFeats&Lemma\\
      \midrule
      Annals & 86.15 & 59.11 & 82.79\\
     Biography & 90.19 & 52.85 & 86.14\\
     Normative & 92.04 & 50.32 & 85.81\\
      Proceedings & 93.18 & 67.12 & 79.82\\
      Science & 75.35 & 51.88 & 96.45\\     
      \bottomrule

\end{tabular}
\caption{The performance of the model pre-trained on all UD corpora evaluated on the \textit{eFontes} data}
 \end{center}
\end{table}

==> tables/confusion_lemmas_all.tex <==
\begin{table}[bp]
\caption{20 most confused lemmas}
\begin{tabular}{lllllr}
category & gold\_upos & gold\_form & gold\_lemma & system\_lemma & count \\
Trial & SYM & */* & */* & + & 46 \\
Biography & NOUN & domine & domina & dominus & 43 \\
Biography & PUNCT & ; & \; & ; & 22 \\
Trial & PROPN & Iohannes & iohannes & johannes & 21 \\
Trial & ADJ & bannitum & bannitus & bannio & 17 \\
Trial & NOUN & marcis & marca & marcus & 17 \\
Trial & PROPN & Nicolao & nicolaus & nicolaum & 17 \\
Trial & PROPN & Nicolaum & nicolaus & nicolaum & 17 \\
Trial & VERB & Veniens & uenio & venio & 17 \\
Trial & NOUN & solucio & solutio & solucium & 12 \\
Biography & VERB & cepit & coepi & capio & 12 \\
Trial & PROPN & Mathias & mathias & mathia & 11 \\
Biography & DET & quod & qui & quod & 10 \\
Biography & PROPN & Kincze & kinga & cincza & 10 \\
Trial & NUM & IIII & IIII & iiii & 9 \\
Biography & ADV & graviter & grauiter & graviter & 9 \\
Trial & ADJ & banitum & bannitus & bano & 8 \\
Trial & NOUN & eternum & aeternum & aeternus & 8 \\
Trial & ADJ & iuste & iustus & iuste & 7 \\
Trial & NOUN & vicinus & uicinus & vicinus & 7 \\
\end{tabular}
\end{table}

==> tables/confusion_lemmas_genre.tex <==
\begin{table}[!ht]
\caption{10 most confused lemmas: Trial}
\begin{tabular}{llllr}
gold
upos & gold
form & gold
lemma & system
lemma & count \\
SYM & */* & */* & + & 46 \\
PROPN & Iohannes & iohannes & johannes & 21 \\
ADJ & bannitum & bannitus & bannio & 17 \\
NOUN & marcis & marca & marcus & 17 \\
PROPN & Nicolao & nicolaus & nicolaum & 17 \\
PROPN & Nicolaum & nicolaus & nicolaum & 17 \\
VERB & Veniens & uenio & venio & 17 \\
NOUN & solucio & solutio & solucium & 12 \\
PROPN & Mathias & mathias & mathia & 11 \\
NUM & IIII & IIII & iiii & 9 \\
\end{tabular}
\end{table}

\begin{table}[!ht]
\caption{10 most confused lemmas: Science}
\begin{tabular}{llllr}
gold
upos & gold
form & gold
lemma & system
lemma & count \\
DET & que & qui & que & 6 \\
NOUN & ypothesi & hypothesis & ipothesium & 6 \\
NOUN & Speras & sphaera & spera & 4 \\
ADJ & equidistans & aequidistans & equidisto & 3 \\
ADJ & equidistantes & aequidistans & equidisto & 3 \\
ADV & seinvicem & seinuicem & seinvicem & 3 \\
VERB & dividit & diuido & divido & 3 \\
ADJ & concavam & concauus & concava & 2 \\
ADJ & convexam & conuexus & convexus & 2 \\
ADV & econtrario & econtrario & econtrarius & 2 \\
\end{tabular}
\end{table}

\begin{table}[!ht]
\caption{10 most confused lemmas: Normative}
\begin{tabular}{llllr}
gold
upos & gold
form & gold
lemma & system
lemma & count \\
NOUN & excommunicacionis & excommunicatio & excommunicacio & 6 \\
VERB & volumus & uolo & volo & 6 \\
ADJ & sinodali & synodalis & senodalis & 5 \\
NOUN & ordinaciones & ordinatio & ordinacio & 5 \\
NOUN & decimarum & decima & decimus & 3 \\
ADJ & Vagus & uagus & vagus & 2 \\
ADJ & diocesani & dioecesanus & diocesanus & 2 \\
ADJ & effrenata & effrenatus & effreno & 2 \\
ADJ & salubria & saluber & salubris & 2 \\
ADV & cicius & cito & ciciter & 2 \\
\end{tabular}
\end{table}

\begin{table}[!ht]
\caption{10 most confused lemmas: Chronicle}
\begin{tabular}{llllr}
gold
upos & gold
form & gold
lemma & system
lemma & count \\
PROPN & Slezie & silesia & slecia & 7 \\
PUNCT & ; & \; & ; & 4 \\
NOUN & Kal. & kalendae & kal. & 3 \\
PROPN & Bohemie & bohemia & bohemias & 3 \\
PROPN & Bolezlaus & boleslaus & bolezlaus & 3 \\
ADJ & valida & ualidus & validus & 2 \\
NOUN & castra & castrum & castra & 2 \\
NOUN & conversionis & conuersio & conversio & 2 \\
NOUN & ventus & uentus & ventus & 2 \\
PROPN & Heinricus & henricus & heinricus & 2 \\
\end{tabular}
\end{table}

\begin{table}[!ht]
\caption{10 most confused lemmas: Biography}
\begin{tabular}{llllr}
gold
upos & gold
form & gold
lemma & system
lemma & count \\
NOUN & domine & domina & dominus & 43 \\
PUNCT & ; & \; & ; & 22 \\
VERB & cepit & coepi & capio & 12 \\
DET & quod & qui & quod & 10 \\
PROPN & Kincze & kinga & cincza & 10 \\
ADV & graviter & grauiter & graviter & 9 \\
NOUN & villam & uilla & villa & 7 \\
NOUN & votum & uotum & votum & 7 \\
VERB & ceperunt & coepi & capio & 7 \\
NOUN & factum & factum & facio & 6 \\
\end{tabular}
\end{table}

==> tables/cross_validation.tex <==
\begin{table}[!ht]
\begin{center}
\begin{tabular}{@{}lrrr@{}}

      \toprule
      Genre&UPOS&UFeats&Lemma\\
      \midrule
      Proceedings & 94.97 & 87.67 & 83.17\\
      Science & 79.61 & 78.60 & 96.35\\
     Annals & 96.20 & 81.45 & 86.82\\
     Biography & 96.10 & 83.86 & 88.12\\
     Normative & 96.10 & 84.86 & 88.37\\
      \bottomrule

\end{tabular}
\caption{Cross-validation results}
 \end{center}
\end{table}
